Knowledge Graphs for Multilingual Language Translation and Generation

The Natural Language Processing (NLP) community has recently seen outstanding progress, catalysed by the release of different Neural Network (NN) architectures. Neural-based approaches have proven effective by significantly increasing the output quality of a large number of automated solutions for NLP tasks (Belinkov and Glass, 2019). Despite these notable advancements, dealing with entities still poses a difficult challenge as they are rarely seen in training data. Entities can be classified into two groups, i.e., proper nouns and common nouns. Proper nouns are also known as Named Entities (NE) and correspond to the name of people, organizations, or locations, e.g., John, WHO, or Canada. Common nouns describe classes of objects, e.g., spoon or cancer. Both types of entities can be found in a Knowledge Graph (KG). Recent work has successfully exploited the contribution of KGs in NLP tasks, such as Natural Language Inference (NLI) (KM et al.,2018) and Question Answering (QA) (Sorokin and Gurevych, 2018). Only a few works had exploited the benefits of KGs in Neural Machine Translation (NMT) when the work presented herein began. Additionally, few works had studied the contribution of KGs to Natural Language Generation (NLG) tasks. Moreover, the multilinguality also remained an open research area in these respective tasks (Young et al., 2018). In this thesis, we focus on the use of KGs for machine translation and the generation of texts to deal with the problems caused by entities and consequently enhance the quality of automatically generated texts.

==> appendices/signatures/sign.tex <==
%\newcommand*\rot{\multicolumn{1}{R{60}{1em}}}% no optional argument here, please
%\chapter*{PUBLICATIONS}
%	\thispagestyle{empty}

% \includepdf[pages=1,pagecommand={\section{\label{appendix:MAG}}}]{appendices/papers/MAG/MAG_to_K_CAP.pdf}
% \includepdf[pages=2-,pagecommand={}]{appendices/papers/MAG/MAG_to_K_CAP.pdf}
\includepdf[pages=1,pagecommand={},trim=0mm 20mm 0mm 0mm]{appendices/signatures/MAG_signed_new.pdf}
\includepdf[pages=1,pagecommand={},trim=0mm 20mm 0mm 0mm]{appendices/signatures/MAG40_signed_new.pdf}

% \section*{MAG: A Multilingual, Knowledge-base Agnostic and Deterministic Entity Linking Approach}
% \large{\textbf{Conference:} K-CAP - Knowledge Capture Conference} \\
% \large{\textbf{Core:} A} \\
% \large{\textbf{Year:} 2017}
% \bigskip
% \bigskip
% \bigskip
% \begin{table*}[htb!]
% \setlength\tabcolsep{10pt}
% \small
% \centering
% %\caption{Fine-grained micro F1 evaluation.}
% \label{tab:signatures}
% \begin{tabular}{@{} lcl@{}}
% \toprule
% Authors & Contribution & Nature of Contributions\\
% \midrule
% Diego Moussallem & 80{\%} & Design of the solution; Data collection; Implementation; \\
% & & Interpretation of results; Drafting and writing of the manuscript \\
% Ricardo Usbeck & 10{\%} & Design of the solution; Drafting and revision of the manuscript \\
% Michael Röder & 5{\%} & Design of the solution; Drafting and revision of the manuscript \\
% Axel-Cyrille Ngonga Ngomo & 5 {\%} & Design of the solution; Drafting and revision of the manuscript \\
% \bottomrule
% \end{tabular}
% \end{table*}
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \begin{center}
% 	\begin{tabular}{l p{0.1\textwidth} r}
% 		\cline{1-1} \cline{3-3}
% 		\begin{minipage}[t]{0.4\textwidth}
% 			\centering
% 				Diego Moussallem
% 		\end{minipage}
% 		&&
% 		\begin{minipage}[t]{0.4\textwidth}
% 			\centering
%                 Ricardo Usbeck
% 		\end{minipage}
% 	\end{tabular}
% \end{center}
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \begin{center}
% 	\begin{tabular}{l p{0.1\textwidth} r}
% 		\cline{1-1} \cline{3-3}
% 		\begin{minipage}[t]{0.4\textwidth}
% 			\centering
% 				Michael Röder
% 		\end{minipage}
% 		&&
% 		\begin{minipage}[t]{0.4\textwidth}
% 			\centering
%                 Axel-Cyrille Ngonga Ngomo
% 		\end{minipage}
% 	\end{tabular}
% \end{center}

% \vspace*{\fill}
% \pagebreak

% \section*{Entity Linking in 40 Languages Using MAG}
% \large{\textbf{Conference:} ESWC - Extended Semantic Web Conference} \\
% \large{\textbf{Core:} A} \\
% \large{\textbf{Year:} 2018}
% \bigskip
% \bigskip
% \bigskip
% \begin{table*}[htb!]
% \setlength\tabcolsep{10pt}
% \small
% \centering
% %\caption{Fine-grained micro F1 evaluation.}
% \begin{tabular}{@{} lcl@{}}
% \toprule
% Authors & Contribution & Nature of Contributions\\
% \midrule
% Diego Moussallem & 80{\%} & Design of the solution; Data collection; Implementation; \\
% & & Interpretation of results; Drafting and writing of the manuscript \\
% Ricardo Usbeck & 10{\%} & Design of the solution; Drafting and revision of the manuscript \\
% Michael Röder & 5{\%} & Design of the solution; Drafting and revision of the manuscript \\
% Axel-Cyrille Ngonga Ngomo & 5 {\%} & Design of the solution; Drafting and revision of the manuscript \\
% \bottomrule
% \end{tabular}
% \end{table*}
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \begin{center}
% 	\begin{tabular}{l p{0.1\textwidth} r}
% 		\cline{1-1} \cline{3-3}
% 		\begin{minipage}[t]{0.4\textwidth}
% 			\centering
% 				Diego Moussallem
% 		\end{minipage}
% 		&&
% 		\begin{minipage}[t]{0.4\textwidth}
% 			\centering
%                 Ricardo Usbeck
% 		\end{minipage}
% 	\end{tabular}
% \end{center}
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \begin{center}
% 	\begin{tabular}{l p{0.1\textwidth} r}
% 		\cline{1-1} \cline{3-3}
% 		\begin{minipage}[t]{0.4\textwidth}
% 			\centering
% 				Michael Röder
% 		\end{minipage}
% 		&&
% 		\begin{minipage}[t]{0.4\textwidth}
% 			\centering
%                 Axel-Cyrille Ngonga Ngomo
% 		\end{minipage}
% 	\end{tabular}
% \end{center}

% \vspace*{\fill}
% \pagebreak
\includepdf[pages=1,pagecommand={},trim=0mm 20mm 0mm 0mm]{appendices/signatures/RDF2PT_signed_new.pdf}
% \section*{RDF2PT: Generating Brazilian Portuguese Texts from RDF Data}
% \large{\textbf{Conference:} LREC - International Conference on Language Resources and Evaluation} \\
% \large{\textbf{Core:} C} \\
% \large{\textbf{Year:} 2018}
% \bigskip
% \bigskip
% \bigskip
% \begin{table*}[htb!]
% \setlength\tabcolsep{10pt}
% \small
% \centering
% %\caption{Fine-grained micro F1 evaluation.}
% \begin{tabular}{@{} lcl@{}}
% \toprule
% Authors & Contribution & Nature of Contributions\\
% \midrule
% Diego Moussallem & 40{\%} & Design of the solution; Data collection; Implementation; \\
% & & Interpretation of results; Drafting and writing of the manuscript \\
% Thiago Castro Ferreira & 40{\%} & Design of the solution; Data collection; Implementation; \\
% & & Interpretation of results; Drafting and writing of the manuscript \\
% Marcos Zampieri & 10{\%} & Design of the solution; Data collection; Drafting and \\
% & & revision of the manuscript \\
% Maria Claudia Cavalcanti & 2 {\%} & Design of the solution; Data collection; Revision of the manuscript \\
% Geraldo Xexéo & 2 {\%} & Design of the solution; Data collection; Revision of the manuscript \\
% Mariana Neves & 2 {\%} & Design of the solution; Data collection; Revision of the manuscript \\
% Axel-Cyrille Ngonga Ngomo & 4 {\%} & Design of the solution; Drafting and revision of the manuscript \\
% \bottomrule
% \end{tabular}
% \end{table*}
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \begin{center}
% 	\begin{tabular}{l p{0.1\textwidth} r}
% 		\cline{1-1} \cline{3-3}
% 		\begin{minipage}[t]{0.4\textwidth}
% 			\centering
% 				Diego Moussallem
% 		\end{minipage}
% 		&&
% 		\begin{minipage}[t]{0.4\textwidth}
% 			\centering
%                 Thiago Castro Ferreira
% 		\end{minipage}
% 	\end{tabular}
% \end{center}
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \begin{center}
% 	\begin{tabular}{l p{0.1\textwidth} r}
% 		\cline{1-1} \cline{3-3}
% 		\begin{minipage}[t]{0.4\textwidth}
% 			\centering
% 				Marcos Zampieri
% 		\end{minipage}
% 		&&
% 		\begin{minipage}[t]{0.4\textwidth}
% 			\centering
%                 Maria Claudia Cavalcanti
% 		\end{minipage}
% 	\end{tabular}
% \end{center}
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \begin{center}
% 	\begin{tabular}{l p{0.1\textwidth} r}
% 		\cline{1-1} \cline{3-3}
% 		\begin{minipage}[t]{0.4\textwidth}
% 			\centering
% 				Geraldo Xexéo
% 		\end{minipage}
% 		&&
% 		\begin{minipage}[t]{0.4\textwidth}
% 			\centering
%                 Mariana Neves
% 		\end{minipage}
% 	\end{tabular}
% \end{center}
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \begin{center}
% 	\begin{tabular}{l p{0.1\textwidth} r}
% 		\cline{1-1} %\cline{3-3}
% 		%\begin{minipage}[t]{0.5\textwidth}
% 			\centering
% 				Axel-Cyrille Ngonga Ngomo
% 		%\end{minipage}
% 	   % &&
% 	%	\begin{minipage}[t]{0.0\textwidth}
% 		%	\centering
%               % Axel-Cyrille Ngonga Ngomo
% 	%	\end{minipage}
% 	\end{tabular}
% \end{center}
% \vspace*{\fill}
% \pagebreak
\includepdf[pages=1,pagecommand={},trim=0mm 20mm 0mm 0mm]{appendices/signatures/NeuralREG_signed_new.pdf}

% \section*{NeuralREG: An end-to-end approach to referring expression generation}
% \large{\textbf{Conference:} ACL - Annual Conference of the Association for Computational Linguistics} \\
% \large{\textbf{Core:} A*} \\
% \large{\textbf{Year:} 2018}
% \bigskip
% \bigskip
% \bigskip
% \begin{table*}[htb!]
% \setlength\tabcolsep{10pt}
% \small
% \centering
% %\caption{Fine-grained micro F1 evaluation.}
% \begin{tabular}{@{} lcl@{}}
% \toprule
% Authors & Contribution & Nature of Contributions\\
% \midrule
% Thiago Castro Ferreira & 40{\%} & Design of the solution; Data collection; Implementation; \\
% & & Interpretation of results; Drafting and writing of the manuscript \\
% Diego Moussallem & 40{\%} & Design of the solution; Data collection; Implementation; \\
% & & Interpretation of results; Drafting and writing of the manuscript \\
% Ákos Kádár & 10{\%} & Design of the solution; Drafting and revision of the manuscript \\
% Sander Wubben & 5 {\%} & Design of the solution; Drafting and revision of the manuscript \\
% Emiel Krahmer & 5 {\%} & Design of the solution; Drafting and revision of the manuscript \\
% \bottomrule
% \end{tabular}
% \end{table*}
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \begin{center}
% 	\begin{tabular}{l p{0.1\textwidth} r}
% 		\cline{1-1} \cline{3-3}
% 		\begin{minipage}[t]{0.4\textwidth}
% 			\centering
% 				Thiago Castro Ferreira
% 		\end{minipage}
% 		&&
% 		\begin{minipage}[t]{0.4\textwidth}
% 			\centering
%                 Diego Moussallem
% 		\end{minipage}
% 	\end{tabular}
% \end{center}
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \begin{center}
% 	\begin{tabular}{l p{0.1\textwidth} r}
% 		\cline{1-1} \cline{3-3}
% 		\begin{minipage}[t]{0.4\textwidth}
% 			\centering
% 				Ákos Kádár
% 		\end{minipage}
% 		&&
% 		\begin{minipage}[t]{0.4\textwidth}
% 			\centering
%                 Sander Wubben
% 		\end{minipage}
% 	\end{tabular}
% \end{center}
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \begin{center}
% 	\begin{tabular}{l p{0.1\textwidth} r}
% 		\cline{1-1} %\cline{3-3}
% 		%\begin{minipage}[t]{0.5\textwidth}
% 			\centering
% 				Emiel Krahmer
% 		%\end{minipage}
% 	   % &&
% 	%	\begin{minipage}[t]{0.0\textwidth}
% 		%	\centering
%               % Axel-Cyrille Ngonga Ngomo
% 	%	\end{minipage}
% 	\end{tabular}
% \end{center}

% \vspace*{\fill}
% \pagebreak
\includepdf[pages=1,pagecommand={},trim=0mm 20mm 0mm 0mm]{appendices/signatures/KGNMT_signed_new.pdf}
% \section*{Utilizing Knowledge Graphs for Neural Machine Translation Augmentation}
% \large{\textbf{Conference:} KCAP - Knowledge Capture Conference} \\
% \large{\textbf{Core:} A} \\
% \large{\textbf{Year:} 2019}
% \bigskip
% \bigskip
% \bigskip
% \begin{table*}[htb!]
% \setlength\tabcolsep{10pt}
% \small
% \centering
% %\caption{Fine-grained micro F1 evaluation.}
% \begin{tabular}{@{} lcl@{}}
% \toprule
% Authors & Contribution & Nature of Contributions\\
% \midrule
% Diego Moussallem & 80{\%} & Design of the solution; Data collection; Implementation; \\
% & & Interpretation of results; Drafting and writing of the manuscript \\
% Axel-Cyrille Ngonga Ngomo & 5{\%} & Design of the solution; Drafting and revision of the manuscript \\
% Paul Buitelaar & 5{\%} & Design of the solution; Drafting and revision of the manuscript \\
% Mihael Arcan & 10 {\%} & Design of the solution; Data Collection, Interpretation of Results \\
% & & Drafting and revision of the manuscript \\
% \bottomrule
% \end{tabular}
% \end{table*}
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \begin{center}
% 	\begin{tabular}{l p{0.1\textwidth} r}
% 		\cline{1-1} \cline{3-3}
% 		\begin{minipage}[t]{0.4\textwidth}
% 			\centering
% 				Diego Moussallem
% 		\end{minipage}
% 		&&
% 		\begin{minipage}[t]{0.4\textwidth}
% 			\centering
%                 Axel-Cyrille Ngonga Ngomo
% 		\end{minipage}
% 	\end{tabular}
% \end{center}
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \begin{center}
% 	\begin{tabular}{l p{0.1\textwidth} r}
% 		\cline{1-1} \cline{3-3}
% 		\begin{minipage}[t]{0.4\textwidth}
% 			\centering
% 				Paul Buitelaar
% 		\end{minipage}
% 		&&
% 		\begin{minipage}[t]{0.4\textwidth}
% 			\centering
%                 Mihael Arcan
% 		\end{minipage}
% 	\end{tabular}
% \end{center}

% \vspace*{\fill}
% \pagebreak
\includepdf[pages=1,pagecommand={},trim=0mm 20mm 0mm 0mm]{appendices/signatures/THOTH_signed_new.pdf}
% \section*{THOTH: Neural Translation and Enrichment of Knowledge Graphs}
% \large{\textbf{Conference:} ISWC - International Semantic Web Conference} \\
% \large{\textbf{Core:} A} \\
% \large{\textbf{Year:} 2019}
% \bigskip
% \bigskip
% \bigskip
% \begin{table*}[htb!]
% \setlength\tabcolsep{10pt}
% \small
% \centering
% %\caption{Fine-grained micro F1 evaluation.}
% \begin{tabular}{@{} lcl@{}}
% \toprule
% Authors & Contribution & Nature of Contributions\\
% \midrule
% Diego Moussallem & 80{\%} & Design of the solution; Data collection; Implementation; \\
% & & Interpretation of results; Drafting and writing of the manuscript \\
% Tommaso Soru & 12{\%} & Design of the solution; Data collection; \\
% & & Drafting and writing of the manuscript \\
% Axel-Cyrille Ngonga Ngomo & 8{\%} & Design of the solution; Drafting and revision of the manuscript \\
% \bottomrule
% \end{tabular}
% \end{table*}
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \begin{center}
% 	\begin{tabular}{l p{0.1\textwidth} r}
% 		\cline{1-1} \cline{3-3}
% 		\begin{minipage}[t]{0.4\textwidth}
% 			\centering
% 				Diego Moussallem
% 		\end{minipage}
% 		&&
% 		\begin{minipage}[t]{0.4\textwidth}
% 			\centering
%                 Tommaso Soru
% 		\end{minipage}
% 	\end{tabular}
% \end{center}
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \bigskip
% \begin{center}
% 	\begin{tabular}{l p{0.1\textwidth} r}
% 		\cline{1-1}
%                 Axel-Cyrille Ngonga Ngomo
% 	\end{tabular}
% \end{center}

% \vspace*{\fill}
% \pagebreak

==> chapters/approaches/LIDIOMS/LIDIOMS.tex <==
In this paper, we describe the LIDIOMS data set, a multilingual RDF representation of idioms currently containing five languages: English, German, Italian, Portuguese, and Russian. The data set is intended to support natural language processing applications by providing links between idioms across languages. The underlying data was crawled and integrated from various sources. To ensure the quality of the crawled data, all idioms were evaluated by at least two native speakers. Herein, we present the model devised for structuring the data. We also provide the details of linking LIDIOMS to well-known multilingual data sets such as BabelNet. The resulting data set complies with best practices according to Linguistic Linked Open Data Community.

% \chapter{LIdioms - A Multilingual Linked Idioms Knowledge Graph}

% %\section{Introduction}
% \label{sec:intro_lid}
% Recently, the \ac{LLOD}\footnote{\url{http://linguistics.okfn.org/}} movement has gained significant momentum.
% According to~\cite{mccrae2016open}, a large number of linguistic data sets have been extracted from various sources and been represented as \ac{LD}. This new movement was motivated by the novel capabilities of the \ac{LD} paradigm pertaining to transforming, sharing, and linking linguistic data on the Web~\cite{chiarcos2012linked}. Resources such as dictionaries and knowledge bases are essential in the development of \ac{NLP} systems. However, most of these resources are still bilingual on the \ac{LLOD}. Thus, becoming worthwhile to develop multilingual knowledge bases by reusing these bilingual contents. Multilingualism is important not only for sharing information across Web but also for learning new concepts from other cultures. 

% There are many data sets and linguistic resources available at \ac{LLOD}, however, most of them do not contain much information about \ac{MWE}. \ac{MWE} are known to constitute a difficult problem on a number of \ac{NLP} tasks such as machine translation, language generation, and sentiment analysis/opinion mining. There are different types of \ac{MWE}, according to~\cite{nunberg1994idioms}, \ac{MWE} are categorized as phrase verbs, compounds, fixed expression, semi-fixed expressions, idioms, slang, and others. This work focuses on idioms, a particular type of \ac{MWE}.

% Most idioms are culture-bound and their senses come from particular concepts of everyday life to a given culture. By definition, idioms are a sequence of words whose meaning cannot be derived from the meaning of words that constitute them~\cite{nunberg1994idioms}. 
% %They are essential for any language while also being 
% %For this reason they are one of the most challenging language phenomena to translate. 
% Idioms are generally classified as non-com\-po\-si\-ti\-o\-nal. One of the direct consequences of non-compositionality is the impossibility of translating this kind of word group literally~\cite{nunberg1994idioms} posing challenges to human translators and to machine translation systems. 
% %task for machine translation systems especially if they do not have a cultural dictionary of the source and target languages.

% In this section, we propose LIDIOMS, a multilingual linked data set of idioms in five languages. In LIDIOMS, we do not distinguish between idioms sub-categories and thus work on idioms in general by providing lexical and semantic knowledge on a multilingual basis. The selected languages are English, German, Italian, Portuguese, and Russian. This choice of languages intends to show the possibility of correct translations among idioms independent of their language family, syntax or culture. Additionally, one of the goals of LIDIOMS is to support further investigations of similarity among idioms from different languages.

% In the following, we begin by presenting the data sources that we used for the extraction (\autoref{sec:source}). In \autoref{sec:onto}, we give an overview of the model that underlies our data set. \autoref{sec:generation} depicts the creation process that led to the publication of our data set. 
% In \autoref{sec:linking}, we present our approach to link LIDIOMS internally and externally. Then, we present usage scenarios for our data set in \autoref{sec:uses}. Subsequently, we discuss \ac{LLOD} quality in \autoref{sec:discussion} %and we conclude the paper and provide avenues for future work in \autoref{sec:conclusion}.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Data Sources}
% \label{sec:source}
% In this section, we list the data sources from which LIDIOMS originates, where we describe the data collection process of each data source. In addition, we discuss how we ensure the quality of the collected data.

% \subsection{Data sets}

% We collected a set of \ac{MWE} from the online lexical resources: (1) \emph{Phrase finder}, (2) \emph{Memrise}, (3) \emph{Collins} and (4) \emph{Oxford} dictionaries\footnote{\label{all}All repositories web pages \url{http://faturl.com/repositories/?open}}.
% \emph{Phrase finder} is an online dictionary about idiomatic expressions created by \emph{Gary Martins}~\cite{martin2007phrase} in 1997 for supporting his post-graduate research in computational linguistics.
% \emph{Memrise} is an online course about idiomatic expressions for achieving a native speaker level.
%  \emph{Collins} and \emph{Oxford} provide high quality lexical resources.
%  Therefore, we use them to guarantee the quality of the idioms definitions and also for gathering some additional idioms. \emph{Memrise} and \emph{Oxford} provided idioms in English, German, Italian, and Russian languages, while the idioms in \emph{Phrase finder} and \emph{Collins} are in English. 
%  The Portuguese idioms were initially gathered from \emph{Wikipedia} Portuguese page\footnote{all} but because of the limited number of the available Portuguese idioms in Wikipedia, we asked four native speakers (one from Portugal and the other three from Brazil) to add more Portuguese idioms.
 
% For the sake of clarity pertaining to the copyrights to use the data, \emph{Memrise} and \emph{Collins} granted us a full permission while the others data providers have a free licence policy when to use the data for research purposes.

% \subsection{Data Collection process}
% \label{sec:dataCollectionProcess}

% Using a custom web crawler, we collected the \ac{MWE} from these aforementioned on-line data sources.
% Each of the crawled resources has specific pages about each \ac{MWE}, which ease the configuration of our crawler.
% Note that, all data sources are bilingual but not necessarily including English as one of the involved languages.
% For instance, \emph{Oxford} has idiomatic expressions from Italian to Portuguese. We also noticed that most on-line dictionaries does not correctly categorize \ac{MWE}. For example, in some cases the meaning of \ac{MWE} can
% be deduced from the meaning of their components (e.g. \emph{``by the book"}) while in other cases this is not possible (e.g. \emph{``out of the blue"}). Therefore, \ac{MWE} which can be represented by the meaning of their components should not be into the same category as the others with pragmatic meanings (i.e. non-compositional idioms). 

% Collecting the right idioms was a hard task due to the lack of \ac{MWE} categorization.
% Thus, we carried out the idiom collection manually where we discarded all the entries that were semantically equivalent to their lexical definitions which means to be \emph{not} non-compositional.
% We dubbed this process \emph{pragmatically-based selection}.
% The pragmatically-based selection identified only $50\%$ of the \ac{MWE} retrieved by our crawler as idioms. For instance, the idiom mentioned before \emph{``by the book"} means ``to follow the rules as demand". The meaning of ``book" is ``a stuff which contains information, rules, descriptions, and it can be a manual". Therefore, this \ac{MWE} is deductible from the meaning of each of its components, the meaning gets ``to follow the book's writing". Therefore, it is not considered an idiom, in contrast of the idiom \emph{``out of the blue"} which means ``an event that occurs unexpectedly", the meaning of ``blue" is ``color" then no relationship exists between ``blue" or ``out of" with ``unexpected happening". 

% Moreover, considering that the meaning of idioms may vary according to the geographical location where they are used~\cite{martin2007phrase}. For example, American idioms which come from The United States of America differ from the British idioms which come from United Kingdom. We consider the location of idioms as an important characteristic to be included in LIDIOMS.

% \subsection{Data Evaluation}

% To ensure the quality of the retrieved data, we asked two native speakers and one linguist (per language) to evaluate the extracted idioms and their respective definitions in English.
% For evaluating an idiom, each native speaker separately evaluated the idioms' definition. 
% Idioms with accepted definitions by both evaluators are accepted. Also, idioms with idioms' definitions marked as wrong by both evaluators were discarded.
% In case a mismatch evaluation happens, the idiom was judged by the linguist. 
% This procedure resulted in a manually checked data set containing a large number of idioms as shown in Table~\ref{tbl:gold}. 
% The \emph{Collection} column shows the number of all \ac{MWE} retrieved by our web crawler.
% The \emph{Filter} column shows the number of idioms retrieved based on our pragmatically-based selection, a step which recognizes only idioms among \ac{MWE} (see \autoref{sec:dataCollectionProcess}).
% The \emph{Total} column presents the resulting number of idioms after the manual review process made by the natives and the linguist.


% \begin{table}[htb]
% \begin{tabularx}{0.48\textwidth}{@{}p{0.13\textwidth}p{0.128\textwidth}p{0.1\textwidth}|p{0.5\textwidth}@{}}
%  \toprule
% \textbf{Language} & \textbf{Collection} & \textbf{Filter} & \textbf{Total}\\
% \midrule
%   English & 1230 & 600 & 291 \\
%   Portuguese & 600 & 215 & 114 \\
%   Italian & 500 & 284 & 175\\
%   German & 400 & 245 & 130\\
%   Russian & 220 & 150 & 105\\
%  \bottomrule
% \end{tabularx}
% \caption{Number of idioms retrieved by step}
% \label{tbl:gold}
% \end{table}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Semantic Representation Model}
% \label{sec:onto}

% The representation model of LIDIOMS aims at describing idioms correctly as a sub-type of \ac{MWE} together with their translations and geographical usage area. 
% For this purpose, LIDIOMS data set is based on Ontolex model. We chose the \emph{Ontolex} model because it contains the necessary classes to represent \ac{MWE} and its translations properly. \emph{Ontolex} also reuses the well-known \emph{Lexinfo} ontology which has an essential term type called \texttt{lexinfo:idiom} for representing idioms as one type of \ac{MWE}. 

% We used the core Ontolex's classes to model LIDIOMS, where (1) we use the class \texttt{on\-to\-lex:Le\-xi\-cal\-En\-try} for representing a lexical entry (i.e. a word, a multi-word expression or an affix), (2) the sub-class \texttt{ontolex:Multi\-word\-Ex\-pres\-sion} is used to specify a lexical entry as a multi-word expression, (3) the  \texttt{on\-to\-lex:Le\-xi\-cal\-Con\-cept} class suits perfectly for representing idioms meaning as its formal definition comprises of ``to be a mental abstraction, concept or a thought that can be described by a given collection of senses". (4) the \texttt{on\-to\-lex:Le\-xi\-cal\-Sen\-se} class for lexical sense of an idiom. (5) the \texttt{on\-to\-lex:Form} class describes the written and alternative forms of the entries and (6) \texttt{on\-to\-lex:Lexicon} class is used for representing a collection of lexical entries.

% For translations, \emph{Ontolex} uses the \emph{vartrans} module which connects \texttt{on\-to\-lex:Le\-xi\-cal\-Sense} instances among themselves through \texttt{var\-trans:\-Trans\-la\-tion} class. The \texttt{var\-trans:Trans\-la\-tion} uses the property \texttt{var\-trans:ca\-te\-gory} for describing translations and also representing variations of these translations across entries in the same\footnote{Same entry from a given language with different meanings} or different languages. 
% The \texttt{var\-trans} module was inspired by~\cite{gracia2014enabling} and we also reuse one of its translation categories called \texttt{tr\-cat:cul\-tu\-ral\-Equi\-va\-lent} which represents a translation between two entries that are not semantically but pragmatically equivalent. Note that a cultural translation of an idiom is not a literal translation, rather it represents the specific cultural semantics of that idiom. 

% For the geographical area of idioms, we use the \texttt{lexvo:usedIn} class from the \emph{Lexvo} Ontology~\cite{de2015lexvo}. The geographical area of an idiom is of great importance because the meaning of an idiom can vary in the same language depending on where it is used (diatopic variation). For instance, the Portuguese idiom \emph{``amarrar o burro"}(its literal translation: ``tie the donkey") means ``to relax" in Portugal while in Brazil it means ``to advise someone about future problems from one action". Furthermore, this idiom has also more meanings even within Brazil, for example, ``to be angry when someone does not allow you to do something" that is typical for children. In addition, some idioms are not understood in all countries even sharing the same language. For instance, the Portuguese idiom \emph{``comprei um mamao"} (eng: ``buy a lemon") is used in Brazil but not in Portugal.

% %MZ: I am not sure about this meaning of "amarrar o burro" in Brazilian Portuguese. I think this idiom is used differently according to the region. The only context I would use is "to settle" but I read it can be used as a synonym for "upset". Perhaps we can find another example?

%  In \autoref{fig:modeling}, we present a complete example of a translation of two idioms from Portuguese (``custa os olhos da cara") to English (``arm and a leg") using \emph{vartrans} class  along with the others descriptions modeled by \emph{Ontolex} in LIDIOMS.

%  \begin{figure*}[tb]
%  \centering
%  \includegraphics[width=\textwidth]{figures/ModelingTrNEW.pdf}
%  \caption{RDF representation of translation of two idioms from Portuguese (``Custa os olhos da cara") to English (``arm and a leg") by entries modeled with the LIDIOMS model.}
%  \label{fig:modeling}
%  \end{figure*}

% In order to represent the names of the languages in a unified way, we publish LIDIOMS based on the best practices of the International Organization of Standardization (ISO). Given the fact that Brazilian Portuguese does not have an ISO resource, we chose to use the Brazilian Portuguese DBpedia resource\footnote{\url{http://dbpedia.org/page/Brazilian_Portuguese}} for substituting that missing ISO.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{RDF Generation}
% \label{sec:generation}
% The original idioms were crawled in heterogeneous formats such as CSV, XML, and HTML. 
% To convert the idiom data into RDF, we used \emph{OpenRefine}\footnote{\url{http://openrefine.org/}} together with its RDF extension. The model underlying the RDF conversion relies on the group of patterns to generate linguistic resources as LD recommended by the \ac{BPMLOD} W3C community group\footnote{\url{https://www.w3.org/community/bpmlod/}}. In spite of our work being multilingual, we followed the patterns for bilingual dictionaries\footnote{\url{https://www.w3.org/2015/09/bpmlod-reports/bilingual-dictionaries/}}. We were able to use bilingual patterns because we use English as pivot language given that all the target translations are in English. 
% Thus, the multilingual translations were found by inference relying on the reflexivity property of the \texttt{vartrans:target}. 
% For more details about LIDIOMS see Table~\ref{tbl:tech} and visit LIDIOMS GitLab repository\footnote{\url{https://github.com/dice-group/LIdioms}}.

% \begin{table}[tb]
%  \begin{tabularx}{0.48\textwidth}{@{}p{0.1\textwidth}p{0.38\textwidth}@{}}
%  \toprule
%  \textbf{Name}		  & LIDIOMS\\
%  \textbf{Example}		  & \url{http://lid.aksw.org/en/kill_two_birds_with_one_stone} \\
%  \textbf{Dump}		  & \url{http://lid.tabsolucoes.com/dataset/dump-1-0.tar.gz} \\
%  \textbf{Sparql}		  & \url{http://lid.aksw.org/sparql} \\
%  \textbf{Repository}		  & \url{https://datahub.io/dataset/lidioms} \\
%  \textbf{Ver. Date}		  & 20.04.2017 \\
%  \textbf{Ver.No}		  & 1.0 \\
%  \textbf{License}		  & CC BY-NC-SA 3.0 \\
%  \bottomrule
%  \end{tabularx}
%   \caption{Technical Details LIDIOMS.}
%     \label{tbl:tech}
%  \end{table}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Linking}
% \label{sec:linking}
% In this section, we describe how we link idioms in LIDIOMS internally (i.e. within the data set) and externally (i.e. with other data sets).

% \subsection{Internal linking}

% While most of the definitions of the retrieved idioms were in English ($87\%$), only in a few cases the definition was in another language.
% We then decided to provide the definitions of all idioms in English regardless of the idioms' original language. 
% The other $13\%$ of idioms which had the definitions in another language were translated by a native speaker to English. Therefore, the English definitions became our pivot language, i.e. the idioms' English definitions were used as bridge for the internal linking process across languages. For instance, the \emph{``when pigs fly"} English idiom has the definition ``something that will never happen". In Portuguese, the idiom \emph{``nem que a vaca tussa"} has exactly the same lexical definition, but its literal translation would be ``nor the cow cough". 
% Still, it is valid to decide to link these two idioms internally based on their definitions.
% \autoref{fig:equivalent} illustrates the main idea underlying this work, i.e. the provision of indirect translations (represented by dotted line) of idioms through a pivot language.

% Note that, some idioms have multiple idiomatic equivalents in other languages while others have none.
% However, some idioms have definitions with almost equivalent syntactic structures while the semantics of the definitions are very different. For instance, the English idiom \emph{``Once in a blue moon"} means \emph{``something that happens rarely"} and another English idiom \emph{``When pigs fly"} means \emph{``something that will never happen"}. This kind of phenomena is likely to decrease the quality of an automatic linking process, because current link discovery frameworks~\cite{nentwig2015survey} only support syntax-based string similarities. Given the lack of support of semantic-based string similarity functions, the internal linking was carried out \emph{manually} by the authors and a cross-validation among the natives and linguists were done on this manual internal linking.

% \begin{figure}[htb]
% \centering
% \includegraphics[scale=0.4]{figures/Indirect.pdf}
% \caption{An indirect translation excerpt}
% \label{fig:equivalent}
% \end{figure}

% The \autoref{tbl:trans} shows the number of direct and indirect translations found for the selected idioms per language.

% \begin{table}[!htb]
% \begin{tabularx}{0.48\textwidth}{@{}p{0.1\textwidth}p{0.03\textwidth}p{0.03\textwidth}p{0.03\textwidth}p{0.03\textwidth}p{0.03\textwidth}|p{0.03\textwidth}@{}}
%  \toprule
% & \textbf{EN} & \textbf{PT} & \textbf{IT} & \textbf{DE} & \textbf{RU} & \textbf{Total} \\
% \midrule
%   \textbf{Idioms} & 291 & 114 & 175 & 130 & 105 & 815 \\
%   \midrule
%   \textbf{Translations} & 192 & 79 & 73 & 62 & 82 & 488 \\
%  \bottomrule
% \end{tabularx}
% \caption{Number of idioms and Translations}
% \label{tbl:trans}
% \end{table}

% \subsection{External linking}

% \begin{table*}[!htb]
% \centering
% \small
% \resizebox{\textwidth}{!}{
% \begin{tabularx}{\textwidth}{@{} XXXXXXXX @{}} 
% \toprule
% \textbf{Languages} & \textbf{LIDIOMS} & \textbf{BabelNet Retrieval} & \textbf{BabelNet Accepted} & \textbf{BabelNet Precision} & \textbf{DBnary Retrieval} & \textbf{DBnary Accepted} & \textbf{DBnary Precision}\\
% \midrule
%  English & 291 & 600 & 195 & 0.325 & 362 & 323 & 0.892  \\
%  Portuguese & 114 & 23 & 9 & 0.391 & 26 & 4 & 0.153 \\
%  Italian & 175 & 52 & 33 & 0.634 & 4 & 4 & 1.0  \\
%  German & 130 & 27 & 8 & 0.296 & 45 & 45 & 1.0 \\
%  Russian & 105 & 48 & 16 & 0.333 & 0 & 0 & 0  \\
%  \textbf{Total} & \textbf{815} & \textbf{750} &  \textbf{261} & \textbf{} & \textbf{437} & \textbf{384} &  \\
%  \bottomrule
% \end{tabularx}
% }
% \caption{Number of links and precision values obtained between LIDIOMS and other data sets.}
% \label{tab:stats}
% \end{table*}

% Linking LIDIOMS to other external resources is based on the string similarities between LIDIOMS's resources and the other data sets' resources. The current version of LIDIOMS is linked to two other data sets in order to ensure re-usability and integrability. 

% The first data set we linked to LIDIOMS is \emph{DBnary}. We used the algorithms provided in LIMES~\cite{ngomo2012link,sherif2015semantic} framework which are time-efficient to carry out the DBnary linking tasks. The linking was through \texttt{rdfs:label} property using the \texttt{trigram} similarity with acceptance threshold $0.85$.

% The second data set we linked with LIDIOMS is \emph{BabelNet}. The BabelNet linking process was carried out using the BabelNet API\footnote{\url{http://babelnet.org/guide}} to retrieve senses and definitions. 
% While linking, we noticed that \emph{BabelNet} do not correctly type idioms (more details see Section \ref{sec:discussion}). We thus linked to BabelNet manually by comparing our \texttt{skos:definition} property with the \texttt{bn-lemon:de\-fi\-ni\-tion} property of the BabelNet resources. This task was performed by the same group of linguists previously requested.

% \subsection{Linking Quality}

% In this section, we show and discuss the linking statistics of LIDIOMS with BabelNet and DBnary.

% %Marcos: Uncomment for full paper.

% \autoref{tab:stats} presents the number of links per resource and language in the LIDIOMS data set. Note that all the links were evaluated manually. The \emph{Retrieval} columns show the number of total idioms collected from a given data set and the \emph{Accepted} columns present the number of idioms which were matched exactly as an idiom. We also present the precision achieved by the aforementioned link specifications. 

% \emph{DBnary} has presented a good precision in general. Its lower score only comes from Portuguese and Russian as these languages are a bit exploited by linguistic resources in terms of \ac{MWE} thus containing only few idioms. \emph{DBnary} follows the best practice of publishing linked data which means without any typos in labels (e.g \texttt{rdfs:label}) in contrast of \emph{BabelNet} (see \footnote{\url{http://babelnet.org/rdf/page/once_in_a_blue_moon_r_EN}}. This problem contributes for the lower precision score of \emph{BabelNet} because its API does not handle it instead of LIMES.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Use Cases}
% \label{sec:uses}
% In this section, we outline selected application scenarios for our data set. \autoref{lst:lst2}, \autoref{lst:lst3} and \autoref{lst:lst4} illustrate different facets of how LIDIOMS can support translation use cases. LIDIOMS contains a significant number of instances of concepts, places and translations. Thus, multilingual idioms along with their definitions concerning about a specific information can be easily retrieved from our data set. Moreover, the aligned multilingual representation allows searching for idioms with the same meaning across different languages.

% \subsection{Gathering idioms by definitions}
% The first use case for our data set is exploratory in nature. 
% Machine translation agents are commonly in need of expressions that have a certain meaning. Using a simple SPARQL query over LIDIOMS enables these potential agents to easily find idioms which contain a keyword of choice. 
% For example, \autoref{lst:lst2} shows a SPARQL query for retrieving English, Italian and Russian idioms which contains the verb \emph{``to deceive''} in their definitions. 

% \begin{lstlisting}[label=lst:lst2, float=htb, style=sparql, numbers=left, numberstyle=\tiny, 
% caption=Idioms definitions that contains the same verb in (i) English (ii) Italian and (iii) Russian.]
% SELECT ?label ?definition
% WHERE { 
%         ?idiom rdfs:label ?label.
%         ?idiom ontolex:sense ?sense.
%         ?sense ontolex:isLexicalizedSenseOf ?concept.
%         ?concept skos:definition ?definition.
% FILTER(bif:contains(?definition, "deceive")) .
% FILTER( lang(?label) = "it" || lang(?label) = "en" || lang(?label) = "rus" ).}

% \end{lstlisting}

% \subsection{Idioms usage per area}
% LIDIOMS provides information about the place of usage of each idiom. For instance, the idiom \emph{``it's raining cats and dogs"} has English as its language property and comes from England.
% By being aware of the place of origin of an idiom, translators are now empowered to translate an idiom to the right idiom for a given target group.  
% \autoref{lst:lst3} shows a SPARQL query which retrieves all idioms from England.    

% \begin{lstlisting}[label=lst:lst3, float=htb, style=sparql, numbers=left, numberstyle=\tiny, 
% caption=All idioms coming from England.]
% SELECT ?idiom ?label
% WHERE { 
%   ?idiom rdfs:label ?label;
%              lexvo:usedIn dbr:England .
% }
% \end{lstlisting}
% \subsection{Translating across languages}

% Another important use of LIDIOMS is to retrieve \emph{indirect translations}. By indirect translation we mean a translation which is based on another translation. Nevertheless, the power of RDF representation of LIDIOMS enable the induction of indirect translations through the English translations.
% For example, the SPARQL query in \autoref{lst:lst4} first finds the English translation of the German idiom \emph{"Zwei Fliegen mit einer Klappe schlagen"}, then it retrieves Russian idioms with equivalent English translations.

% \begin{lstlisting}[label=lst:lst4, float=htb, style=sparql, numbers=left, numberstyle=\tiny, 
% caption=Indirect translation.]
% SELECT  ?idiom
% WHERE { 
%   ?i rdfs:label "zwei fliegen mit einer klappe schlagen"@de; 
%       ontolex:sense ?sense.  
%   ?trans vartrans:source ?sense;
%           vartrans:target ?target.
%   ?transind vartrans:target ?target;
%               vartrans:source ?source.
%   ?lex ontolex:sense ?source;
%          rdfs:label    ?idiom.
%  FILTER( lang(?idiom) = "rus" ). 
% }
% \end{lstlisting}

% \subsection{Third-party uses: Retrieving More Information through Links}

% LIDIOMS is linked to other data sets, from which we are able to retrieve additional idiom-related information.
% For example, \autoref{lst:link} shows a SPARQL query for retrieving a given part-of-speech tag of the English idiom \emph{``out of the blue"} from the same resource exists in \emph{DBnary}.

% \begin{lstlisting}[label=lst:link, float=htb, style=sparql, numbers=left, numberstyle=\tiny, 
% caption=Retrieving data from different resources.]
% SELECT ?pos
%     WHERE { 
%       ?idiom rdfs:label "out of the blue"@en;
%               owl:sameAs ?ext_idiom.
%       SERVICE <http://kaiko.getalp.org/sparql> {
%         SELECT ?ext_idiom ?pos
%         WHERE{
%           ?ext_idiom dbnary:partOfSpeech ?pos
%         }
%     }
% }
% \end{lstlisting}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsubsection{Discussion}
% \label{sec:discussion}

% A main limitation in the currently available data sets in \ac{LLOD} is the lack of proper categorization of \ac{MWE}. For example, neither \emph{BabelNet} nor \emph{DBnary} have specific \ac{MWE} types. For instance, in \emph{BabelNet}, some idioms were not typed as lexical entries, we were capable of finding exact matches of many idioms which are included in LIDIOMS but the matches were from other classes such as a film, a book or music album (e.g., ``head over heels" is the label of a film\footnote{\url{http://babelnet.org/rdf/page/s03412613n}}). In order to alleviate this problem, we also tried to filter the idioms by \emph{bn-lemon:synsetType} in BabelNet, however, incorrect types avoided us to link them easily. For example, the idiom ``The Goose That Laid the Golden Eggs" is typed as ``Named Entity" (see http://babelnet.org/\-rdf/page/s032\-00922n), but it should be a concept. Additionally, \autoref{lst:bn_resources} shows an example resource from BabelNet. 

% \begin{lstlisting}[label=lst:bn_resources, float=t, style=sparql, numbers=left, numberstyle=\tiny, 
% caption=Fragment of a \emph{BabelNet} resource.]
% bn:arm_and_a_leg_n_EN
%   a                     lemon:LexicalEntry ;
%   rdfs:label            "arm_and_a_leg"@en ;
%   lemon:canonicalForm   <http://babelnet.org/rdf/arm_and_a_leg_n_EN/canonicalForm> ;
%   lemon:language        "EN" ;
%   lemon:sense           <http://babelnet.org/rdf/arm_and_a_leg_EN/s13676929n> ;
%   lexinfo:partOfSpeech  lexinfo:noun .
   
% \end{lstlisting}

% In \autoref{lst:bn_resources}, the idiom \emph{``arm and a leg"} is represented as a \emph{noun} while it should be firstly represented as a \ac{MWE} or more precisely as an idiom. This lack of accurate categorization of \ac{MWE} makes linking data sources such as LIDIOMS with other resources very difficult. In particular, using declarative link discovery frameworks for computing similarities among \ac{MWE} without the right classification information becomes a slow task which leads to links with a low level of precision.  

% Furthermore, this incomplete categorization exists also in other data sets such as \emph{DBpedia} and \emph{DBnary}. We thus regard LIDIOMS as a first effort towards a better LLOD, where \ac{MWE}s (especially idioms) are represented as such. We envision that this better representation will lead to qualitative linked-data driven \ac{NLP} systems, including but not limited to better \ac{MT} applications.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> glyphtounicode-ntx.tex <==
%%
%%   file:  glyphtounicode-ntx.tex
%%    version 1.02     date:  2019-02-11
%
% Unicode mappings for ntx text/math glyph names
% (c) 2018, 2019  Ross Moore   <ross.moore@mq.edu.au>
%  
% These should be loaded along with the files:
%    glyphtounicode.tex
%    glyphtounicode-cmr.tex
%  when generating files to validate for  PDF/A  and/or Accessibiity (PDF/UA)
%  using  newtxmath.sty   and/or  newtxtext.sty .
%
%% possible corrections - - depends upon usage ???
\begingroup
\let\p\pdfglyphtounicode
\p{slurabove}{2312}%   was  2322 'frown'

%% from TeXGyre fonts
\p{cwm}{200B}%  0-width space
\p{diameter}{2300}%
\p{anglearc}{2222}%
\p{ell}{2113}%
\p{dotbelow}{0323}%
\p{hookabove}{0309}%
%% Private Use  characters
\p{threequartersemdash}{2014}%  was  F6DE
%% from txmia  (and also  txmbia )
\p{g1}{D835 DC54}% 0067
\p{y1}{D835 DC66}% 0079
\p{v1}{D835 DC63}% 0076
\p{w1}{D835 DC64}% 0077
\p{bbA}{D835 DD38}% 
\p{bbB}{D835 DD39}% 
\p{bbC}{2102}% *
\p{bbD}{D835 DD3B}% 
\p{bbE}{D835 DD3C}% 
\p{bbF}{D835 DD3D}% 
\p{bbG}{D835 DD3E}% 
\p{bbH}{210D}% *
\p{bbI}{D835 DD40}% 
\p{bbJ}{D835 DD41}% 
\p{bbK}{D835 DD42}% 
\p{bbL}{D835 DD43}% 
\p{bbM}{D835 DD44}% 
\p{bbN}{2115}% * 
\p{bbO}{D835 DD46}% 
\p{bbP}{2119}% 
\p{bbQ}{211A}% *
\p{bbR}{211D}% *
\p{bbS}{D835 DD4A}% 
\p{bbT}{D835 DD4B}% 
\p{bbU}{D835 DD4C}% 
\p{bbV}{D835 DD4D}% 
\p{bbW}{D835 DD4E}% 
\p{bbX}{D835 DD4F}% 
\p{bbY}{D835 DD50}% 
\p{bbZ}{2124}%  * 
\p{bbk}{D835 DD5C}% 
%% from txsyc  (and also  txbsyc)
\p{nequal}{2260}
\p{npropersubset}{2284}
\p{npropersuperset}{2285}
\p{nelement}{2209}
\p{nowner}{220C}
\p{colonequal}{2254}
\p{equalcolon}{2255}
%% from txbsya
\p{squaresmallsolid}{25A0}
\p{axisshort}{2027}% hyphenation point
\p{arrowaxisright}{27A1}% Dingbat
\p{arrowaxisleft}{2B05}% black arrow
%% from txbsyb
\p{lessornotsimilar}{22E6}
\p{greaterornotsimilar}{22E7}
\p{notsimequal}{2247}
\p{subsetornoteql}{2ACB}
\p{supersetornoteql}{2ACC}
\p{notshortbar}{2016 0337}
\p{notshortparallel}{2AF2}%  ?
\p{barshort}{2758}% ?
\p{parallelshort}{2016}% ?
%% from  txsyc  and  txbsyc 
\p{mapsfrom}{2ADE}% turnstile ?
\p{Mapsto}{27FE}% double arrow
\p{Mapsfrom}{2AE4}% turnstile ?
\p{mmapsto}{2AE6}% turnstile ?
\p{mmapsfrom}{2AE3}% turnstile  ?
\p{Mmapsto}{255E}% turnstile ?
\p{Mmapsfrom}{2AE5}% turnstile ?
\p{medcircle}{25CB}
\p{medbullet}{25CF}
\p{parallel1}{2225}
\p{nparallel}{2226}
\p{nparallel1}{2226 FE01}
\p{colonapprox}{003A 2248}
\p{colonsim}{003A 223C}
\p{coloncolonapprox}{003A 2248}
\p{coloncolonsim}{003A 003A 223C}
\p{doteq}{2250}
\p{multimapinv}{27DC}
\p{multimapboth}{29DF}
\p{solidmultimap}{22B8 FE01}
\p{solidmultimapinv}{27DC FE01}
\p{solidmultimapboth}{29DF FE01}
\p{rsolidmultimapboth}{22B6}
\p{lsolidmultimapboth}{22B7}
\p{forcesextra}{22AB}% turnstile ?
\p{Forcesbar}{22AA}%  turnstile ???
\p{simequal}{2245}
\p{precedesordblequal}{2AB3}
\p{followsordblequal}{2AB4}
\p{notprecedesorsimilar}{22E0}
\p{notfollowsorsimilar}{22E1}
\p{notlessorsimilar}{2274}
\p{notgreaterorsimilar}{2275}
\p{notlessorapproxeql}{2A85 0338}
\p{notgreaterorapproxeql}{2A86 0338}
\p{notprecedesorcurly}{22E0}
\p{notfollowsorcurly}{22E1}
\p{notgreaterorless}{2279}
\p{notlessorgreater}{2278}
\p{notdifference}{224F 0338}
\p{notgeomequivalent}{224E 0338}
\p{notrevsimilar}{223D 0338}
\p{notrevasymptequal}{22CD 0338}
\p{nequal}{2260}
\p{nequivasymptotic}{226D}
\p{nequivalence}{2262}
\p{nsimilar}{2241}
\p{napproxequal}{2249}
\p{npropersubset}{2284}
\p{npropersuperset}{2285}
\p{nlessmuch}{226A 0338}
\p{ngreatermuch}{226B 0338}
\p{notapproxequal}{2249}
\p{notapproxorequal}{224A 0338}
\p{notfollowsorequal}{2AB7 0338}
\p{notprecedesorequal}{2AB8 0338}
\p{notprecedesordblequal}{2AB3 0338}
\p{notfollowsordblequal}{2AB4 0338}
\p{nsimilarequal}{2244}
\p{nelement}{2209}
\p{nowner}{220C}
\p{notsubsetdbl}{22D0 0338}
\p{notsupersetdbl}{22D1 0338}
\p{nsubsetsqequal}{22E2}
\p{nsupersetsqequal}{22E3}
\p{colonequal}{2254}
\p{equalcolon}{2255}
\p{colonbar}{003A 002D}
\p{barcolon}{2239}
\p{Colonequal}{2A74}
\p{Equalcolon}{2255 }
\p{Colonbar}{003A 003A 002D}
\p{Barcolon}{2239 003A}
\p{strict}{297D}%  fish tail
\p{strictinverse}{297C}%  fish tail
\p{strictboth}{297C 297D}%  fish tails
\p{ampersandinv}{214B}
\p{lbag}{27C5}
\p{rbag}{27C6}
\p{lbagbig}{27C5 FE01}
\p{rbagbig}{27C6 FE01}
\p{oless}{29C0}
\p{ogreater}{29C1}
\p{owedge}{2227 20DD}
\p{ovee}{2228 20DD}
\p{circlebar}{233D}%  APL ?
\p{circlebackslash}{2298}
\p{multicloseleft1}{22C9}
\p{multicloseright1}{22CA}
\p{multicloseboth1}{22C8 FE01}
\p{multiopenboth1}{2715 FE01}
\p{multicloseboth}{22C8}
\p{multiopenboth}{2715}
\p{Diamond}{25C7}
\p{Diamondsolid}{25C6}
\p{intersectmulti}{2A44 FE01}%  ???
\p{notsquareimage}{228F 0338}
\p{notsquareoriginal}{2290 0338}
\p{dashedarrowleft}{290E}
\p{dashedarrowright}{290F}
\p{dashedarrowboth}{290E 290F}
\p{squiggleleft}{21DC}
\p{notdblarrowheadright}{2900}
\p{notdblarrowheadleft}{219E 0337}
\p{squareasterisk}{29C6}
\p{squarebackslash}{29C5}
\p{squarebar}{25EB}
\p{squareslash}{29C4}
\p{Wreathproduct}{2240 2240}
\p{lambdaslash}{019B}
\p{lambdabar}{D835 DF06 0335}
\p{club1}{2667}
\p{diamond1}{2666}
\p{heart1}{2665}
\p{spade1}{2664}
\p{Arrownortheast}{21D7}
\p{Arrowsoutheast}{21D8}
\p{Arrownorthwest}{21D6}
\p{Arrowsouthwest}{21D9}
\p{Latticetop}{2AEA}
\p{Perpendicular}{2AEB}
\p{leadstoext}{219D}
\p{leadsto}{301C}%  ???
\p{squareunionmulti}{228E FE01}
\p{squareintersectmulti}{2A4E FE01}
\p{dblbracketleft}{27E6}
\p{dblbracketright}{27E7}
\p{squareright}{25A1 2192}
\p{squareleft}{2190 25A1}
\p{squaredotright}{22A1 2192}
\p{squaredotleft}{2190 22A1}
\p{Diamondright}{25C7 2192}%
\p{Diamondleft}{2190 25C7}
\p{Diamonddotright}{27D0 2192}
\p{Diamonddotleft}{2190 27D0}
\p{squareRight}{25A1 21D2}
\p{squareLeft}{21D0 25A1}
\p{squaredotRight}{22A1 21D2}
\p{squaredotLeft}{21D0 22A1}
\p{DiamondRight}{25C7 21D2}
\p{DiamondLeft}{21D0 25C7}
\p{DiamonddotRight}{27D0 21D2}
\p{DiamonddotLeft}{21D0 27D0}
\p{Diamonddot}{27D0}
\p{circleright}{25CB 2192}
\p{circleleft}{2190 25CB}
\p{circledotright}{2299 2192}
\p{circledotleft}{2190 2299}
\p{opentrans}{260D FE01}%  ???
\p{solidtrans}{2051 20D2}%  ???
\p{topsolidtrans}{2AF1 FE01}%  ???
\p{topopentrans}{27DF FE01}% ???

%% from txsys
\p{arcwide}{0361}
\p{arcwider}{0361 FE01}% variants according size
\p{arcwiderr}{0361 FE02}% .. .. 
\p{arcwidest}{0361 FE03}% .. .. 
\p{arcwideult}{0361 FE04}% .. .. 
\p{barbar}{0304 0304}
\p{barhat}{0304 0303}
\p{bartilde}{0304 0302}
\p{bulletS}{25C5}
\p{bulletSS}{2022}
\p{bulletSSS}{2219}
\p{cdotB}{00B7}
\p{cdotBB}{22C5}
\p{ddddot}{20DC}
\p{ddddotacc}{20DC}
\p{dddot}{20DB}
\p{dddotacc}{20DB}
\p{ddotacc}{0308}
\p{dotacc}{0307}
\p{emptysetAlt}{2300}
\p{emptysetAlt2}{2205}
\p{harpoonacc}{20D2}
\p{hatbar}{0303 0304}
\p{hathat}{0303 0303}
\p{hattilde}{0303 0302}
\p{lharpoonacc}{20D0}
\p{lrharpoonacc}{20E1}
\p{lrvec}{20E1}
\p{lvec}{20D6}
\p{nexists}{2204}
\p{oarcwide}{0361 0350}% try to add upper arrow-tip
\p{oarcwider}{0361 FE01 0350}%  .. .. 
\p{oarcwiderr}{0361 FE02 0350}%  .. .. 
\p{oarcwidest}{0361 FE03 0350}%  .. .. 
\p{oarcwideult}{0361 FE04 0350}%  .. .. 
\p{prime2}{02B9}
\p{smcompB}{25CB}
\p{tildebar}{0302 0304}
\p{tildehat}{0302 0303}
\p{tildetilde}{0302 0302}
\p{rvec}{20D7}
\p{vec}{20D7}
%  from txex-bar, txbex-bar
\p{angleleftbigx}{27E8 FE01}% variants according size
\p{anglerightbigx}{27E9 FE01}
\p{braceleftbigx}{007B FE01}
\p{bracerightbigx}{007D FE01}
\p{bracketleftbigx}{005B FE01}
\p{bracketrightbigx}{005D FE01}
\p{ceilingleftbigx}{2308 FE01}
\p{ceilingrightbigx}{2309 FE01}
\p{floorleftbigx}{230A FE01}
\p{floorrightbigx}{230B FE01}
\p{parenleftbigx}{0028 FE01}
\p{parenrightbigx}{0029 FE01}
\p{bardblex}{2225 FE01}
\p{bardblexbigx}{2225 FE02}
\p{barex}{007C FE01}
\p{barexbigx}{007C FE01}
\p{bracehext}{02C9}%  use a macron for horizontal spacing !!
\p{grouphtipdownleft}{02CA}%  use spacing modifiers to simulate the overbrace 
\p{grouphtipdownright}{02CB}%  .. ..
\p{grouphtipupleft}{02CF}%  use spacing modifiers to simulate the underbrace
\p{grouphtipupright}{02CE}%  .. ..
\p{groupatipdownleft}{1DFE 02CA}%  include an arrow-tip
\p{groupatipdownright}{02CB 0350}%  include an arrow-tip
\p{groupatipupleft}{02F1 02CF}%  include an arrow-tip
\p{groupatipupright}{02CE 02F2}%  include an arrow-tip
\p{parenleftbtA}{239D}
\p{parenleftexA}{239C}
\p{parenlefttpA}{239B}
\p{parenrightbtA}{23A0}
\p{parenrightexA}{239F}
\p{parenrighttpA}{239E}
\p{hat4}{0302 FE04}% variants according to width
\p{hat5}{0302 FE05}%   .. .. ..
\p{hat6}{0302 FE06}%   .. .. ..
\p{tilde4}{0303 FE04}% variants according to width
\p{tilde5}{0303 FE05}%   .. .. ..
\p{tilde6}{0303 FE06}%   .. .. ..
% from   txexs  
\p{cupdottext}{2A03}
\p{cupdotdisplay}{2A03}
\p{dblbracketleftbig}{27E6 FE01}% variants according to size
\p{dblbracketleftbigg}{27E6 FE02}% .. ..
\p{dblbracketleftBig}{27E6 FE03}% .. ..
\p{dblbracketleftBigg}{27E6 FE04}% .. ..
\p{dblbracketleftbt}{23A5 23A3}% gives a solid v-line before bracket pieces
\p{dblbracketleftex}{23A5 23A2}%    double lines
\p{dblbracketlefttp}{23A5 23A1}%    upper left-bracket pieces
\p{dblbracketrightbig}{27E6 FE01}% variants according to size
\p{dblbracketrightbigg}{27E6 FE02}% .. ..
\p{dblbracketrightBig}{27E6 FE03}% .. ..
\p{dblbracketrightBigg}{27E6 FE04}% .. ..
\p{dblbracketrightbt}{23A6 23A2}% gives a solid v-line after bracket pieces
\p{dblbracketrightex}{23A5 23A2}%    double lines
\p{dblbracketrighttp}{23A4 23A2}%    upper right-bracket pieces
\p{intersectionsqtext}{2A05 FE01}
\p{intersectionsqdisplay}{2A05 FE01}
\p{intersectmultitext}{2A44 FE00}%  variant of  'intersect with logical and'
\p{intersectmultidisplay}{2A44 FE00}%  variant of  'intersect with logical and'
\p{intersectsqmultitext}{2A05 FE00}%  variant of  'n-ary square intersection'
\p{intersectsqmultidisplay}{2A05 FE00}%  variant of  'n-ary square intersection'
\p{lbagbig}{27C5 FE01}% variants according to size
\p{lbagbigg}{27C5 FE02}% .. .. 
\p{lbagBig}{27C5 FE03}% .. ..
\p{lbagBigg}{27C5 FE04}% .. ..
\p{lbagBiggg}{27C5 FE05}% .. ..
\p{lbagBigggg}{27C5 FE06}% .. ..
\p{lbagBiggggg}{27C5 FE07}% .. ..
\p{rbagbig}{27C6 FE01}% variants according to size
\p{rbagbigg}{27C6 FE02}% .. ..
\p{rbagBig}{27C6 FE03}% .. ..
\p{rbagBigg}{27C6 FE04}% .. ..
\p{rbagBiggg}{27C6 FE05}% .. ..
\p{rbagBigggg}{27C6 FE06}% .. ..
\p{rbagBiggggg}{27C6 FE07}% .. ..
\p{producttext1}{2715}%  Dingbat multiply symbol
\p{productdisplay1}{2715}%  Dingbat multiply symbol
\p{raisedsquare}{2E0B}%  not used, for 'missing' (.notdef) symbol ???
\p{unionsqmultitext}{2A04 FE00}%  variant of non-square union
\p{unionsqmultidisplay}{2A04 FE00}%  variant of non-square union
%  T1-encoding
\p{perthousandzero}{2080}%  use subscript 0
%  ntxsyralt , fourier-ml ,  fourier-ms, . . .
\p{kappa1}{D835 DF18}
\p{kappa1up}{03F0}
\p{rho2}{03F1}
\p{partialdiff1}{D835 DF15}
\p{pi2}{03D6}
\p{emptysetstress}{2205}
\p{mapstochar}{21A6}%  ???
\p{radicallow}{23B7}% 221A ???
%  fxlri-7alt  (and  fxlri-5alt etc. )
\p{J.alt}{D835 DE11}
\p{g.alt}{D835 DE28}
\p{v.alt}{D835 DE37}
\p{w.alt}{D835 DE38}
\p{y.alt}{D835 DE3A}
%  rtxbmi-rev , rtxbmi5-rev , rtxbmi7-rev 
\p{harpoonleftup}{21BC}% was incorrectly {21BF}
\p{harpoonrightup}{21C0}% was incorrectly {21BE}
\p{harpoonleftdown}{21BD}% was incorrectly {21C3}
\p{harpoonrightdown}{21C1}% was incorrectly {21C2}
\p{hookleftchar}{02D2}
\p{hookrightchar}{02D3}
%  fourier and other arrows and math symbols
\p{dotaccent}{0307}
\p{geqslant}{2A7E}
\p{leqslant}{2A7D}
\p{notgeqslant}{2A7E 0338}
\p{notleqslant}{2A7D 0338}
\p{parallelslanted}{2225}
\p{notparallelslanted}{2226}
\p{vDash}{22A8}
\p{notvDash}{22AD}
\p{blacktriangleleft}{25B6}
\p{blacktriangleright}{25C0}
\p{hslash}{210F}
\p{notexists}{2204}
\p{bartriple}{2AF4}
\p{bracketdoubleleft}{27E6}
\p{bracketdoubleright}{27E7}
\p{varsubsetneq}{228A}
\p{subsetneqq}{2ACB}
\p{notowner}{220C}
\p{smallsetminus}{2216}% ???
\p{swords}{2694}
\p{swordsdown}{2694}%  !!! 
\p{curvearrowleft}{21B6}
\p{curvearrowright}{21B7}
\p{leftleftarrows}{21C7}
\p{rightrightarrows}{21C9}
\p{barcino}{1F60E}% !!!
\p{apple}{1F34E}%  was {F8FF}
\p{arrowhorizex}{23AF}% was {F8E7}
\p{arrowvertex}{23D0}% was {F8E6}
\p{integralex}{23AE}% was {F8F5}
\p{radicalex}{23AF}%  ???  was {F8E5}


\endgroup

==> shthesis-pre.tex <==


